A High Efficiency Photon Veto for the Light Dark Matter eXperiment

Fixed-target experiments using primary electron beams can be powerful discovery tools for light dark matter in the sub-GeV mass range. The Light Dark Matter eXperiment (LDMX) is designed to measure missing momentum in high-rate electron fixed-target reactions with beam energies of 4 GeV to 16 GeV. A prerequisite for achieving several important sensitivity milestones is the capability to efficiently reject backgrounds associated with few-GeV bremsstrahlung, by twelve orders of magnitude, while maintaining high efficiency for signal. The primary challenge arises from events with photo-nuclear reactions faking the missing-momentum property of a dark matter signal. We present a methodology developed for the LDMX detector concept that is capable of the required rejection. By employing a detailed GEANT4-based model of the detector response, we demonstrate that the sampling calorimetry proposed for LDMX can achieve better than $10^{-13}$ rejection of few-GeV photons. This suggests that the luminosity-limited sensitivity of LDMX can be realized at 4 GeV and higher beam energies.

==> sections/signaleff.tex <==


%\rpt{update numbers/plot/table}


%
%
%

The signal efficiency after applying all background rejection cuts discussed 
above is 
%shown in Fig.~\ref{fig:sig_eff} and 
summarized for three \aprime mediators in Tab.~\ref{tab:sig_eff}.  
After all cuts, the signal efficiency is approximately 50\% in the mass range from 10\,MeV to 0.5\,GeV. 
This efficiency is used in the calculation of the 
expected sensitivity described in the next section.

%%%%%%%%%%%%%%
%   Figure   %
%%%%%%%%%%%%%%
%\begin{figure}[!ht] 
%    \centering
%    \includegraphics[width=.7\textwidth]{figures/sig_efficiency.pdf}
%    \caption{The signal efficiency after applying all background rejection 
%             cuts.} 
%    \label{fig:sig_eff}
%\end{figure}  
%%%%%%%%%%%%%%
%   Figure   %
%%%%%%%%%%%%%%

\begin{table}[!b]
    \centering
    \begin{tabular}{ l | c c c  } 
        
        \multicolumn{4}{c}{Signal Cutflow} \\ [0.5ex]
        \hline\hline
        & \textbf{1 MeV} & \textbf{100 MeV} & \textbf{1000 MeV} \\ [0.5ex]
        \hline
        & \multicolumn{3}{c}{$\epsilon$ (\%)} \\
        \hline
        Trigger requirement & 57 & 91 & 97 \\ 
        %Recoil $e^-$ in \ecal \footnote{Events where the recoil misses the \ecal are the subject of a separate, ongoing analysis.  We expect comparable or better performance in that complementary sample.}  & ? & ? \\ 
        %Triggered Events & ? & ?\\ 
        \ecal Shower-Profile BDT         & 38 & 79 & 82 \\ 
        \hcal Max PE $<3$                & 37 & 76 & 63 \\ 
        Single track with $p < 1.2$ \GeV & 31 & 56 & 34 \\ 
        Recoil activity Cut              & 30 & 54 & 33 \\ 
        \ecal activity cut               & 29 & 53 & 32 \\ 
        Tagger tracker activity cut      & 29 & 51 & 31 \\ 
        \hline
    \end{tabular}
    \caption{Signal efficiency for 1, 100 and 1000 MeV after successive 
             background rejection cuts.}
    \label{tab:sig_eff}
\end{table}
%\ednote{Talk about varying the target thickness, not necessarily with dedicated studies?}

